Political audience diversity and news reliability in algorithmic ranking

Newsfeed algorithms frequently amplify misinformation and other low-quality content. How can social media platforms more effectively promote reliable information? Existing approaches are difficult to scale and vulnerable to manipulation. In this paper, we propose using the political diversity of a website's audience as a quality signal. Using news source reliability ratings from domain experts and web browsing data from a diverse sample of 6,890 U.S. citizens, we first show that websites with more extreme and less politically diverse audiences have lower journalistic standards. We then incorporate audience diversity into a standard collaborative filtering framework and show that our improved algorithm increases the trustworthiness of websites suggested to users -- especially those who most frequently consume misinformation -- while keeping recommendations relevant. These findings suggest that partisan audience diversity is a valuable signal of higher journalistic standards that should be incorporated into algorithmic ranking decisions.

==> titlepage_misinforeview.tex <==
\title{Audience diversity may serve as a valuable signal for social media platforms to detect high quality news}

\author{}

\date{March 2020}

\maketitle

\begin{abstract}
An analysis of news source reliability ratings compiled by domain experts and web browsing histories from a diverse sample of 19,282 U.S. citizens suggest that using political diversity of online audience as a metric can help social media platforms identify high-quality media outlets. Our findings show an algorithmic approach to improving news content circulated online.    
\end{abstract}


% Research shows that people have strong preferences for pro-attitudinal content. These tendencies are exacerbated by social media platforms, which often amplify low-quality content because it generates high levels of engagement among like-minded audiences. 

% Whole article should be <=3000 words 

\section*{Research Question} 
Can the political diversity of a media outlet's audience tell us anything about its quality?


\section*{Summary of Findings}
\begin{itemize}
    \item Partisan audience diversity is a valuable signal of higher journalistic standards that should be incorporated into algorithmic ranking decisions. Popularity, measured by the number of access a website receives, does not predict higher quality journalistic standards.
    \item Observational results indicate that sites with more extreme and less politically diverse audiences have lower journalistic standards.
    \item We also use k-fold cross-validation to demonstrate that incorporating audience diversity into a model of news quality better identifies high quality websites than a model using audience size alone.
    \item  To understand the real-world implications of these finding, we incorporate audience diversity into a collaborative filtering recommendation system and show that our improved algorithm increases trustworthiness of websites suggested to users.
    
\end{itemize}

